TrajectoryNet: A Dynamic Optimal Transport Network for Modeling Cellular Dynamics

It is increasingly common to encounter data from dynamic processes captured by static cross-sectional measurements over time, particularly in biomedical settings. Recent attempts to model individual trajectories from this data use optimal transport to create pairwise matchings between time points. However, these methods cannot model continuous dynamics and non-linear paths that entities can take in these systems. To address this issue, we establish a link between continuous normalizing flows and dynamic optimal transport, that allows us to model the expected paths of points over time. Continuous normalizing flows are generally under constrained, as they are allowed to take an arbitrary path from the source to the target distribution. We present TrajectoryNet, which controls the continuous paths taken between distributions to produce dynamic optimal transport. We show how this is particularly applicable for studying cellular dynamics in data from single-cell RNA sequencing (scRNA-seq) technologies, and that TrajectoryNet improves upon recently proposed static optimal transport-based models that can be used for interpolating cellular distributions.

==> sections/1_old_introduction.tex <==
In data science we are often confronted with cross-sectional samples of time-varying phenomenon, especially in biomedical data. Examples include health measurements of different age cohorts~\cite{oeppen_broken_2002}, or disease measurements at different stages of disease severity~\cite{waddington_epigenotype_1942}. Extracting the longitudinal dynamics of development or disease from static snapshot measurements can be challenging as straightforward methods of interpolation do not work. Further exacerbating this problem is the fact that the same entities are often not measured at each time, resulting in a lack of point-to-point correspondences. Here, we propose to formulate this problem as one of optimal, unbalanced dynamic transport, where the goal is to transport entities from one cross sectional measurement to the next using efficient and smooth paths.  Our main contribution is to establish a link between {\em continuous normalizing flows} (CNF)~\cite{grathwohl_ffjord_2019} and dynamic optimal transport~\cite{benamou_computational_2000}. This link allows us to efficiently solve the transport problem using a Neural ODE framework~\cite{chen_neural_2018}. To our knowledge, TrajectoryNet is the first method to consider the specific paths taken by a CNF between distributions. Although, widely applicable, we focus our results on the problem of understanding cellular differentiation from snapshot scRNA-seq measurements. %This model is particularly well suited to this data as we are measuring a non-linear dynamic system with cross-sections of a population at relatively few discrete timepoints.

Single cell RNA sequencing~\cite{macosko_highly_2015} is a relatively new technology that has made it possible for scientists to randomly sample the entire transcriptome, i.e, 20-30 thousand species mRNA molecules representing transcribed genes of the cell, thereby elucidating very precise information about the identity of the cell based on transcription factors, surface marker expression, extra cellular communication, signaling, cell cycle and many other facets of cellular behavior. In particular, this technology can be used to learn how cells differentiate from one state to another: for example, from embryonic stem cells to specified lineages such as neuronal or cardiac, or from undifferentiated neuronal progenitors to mature frontal cortex neurons. However, hampering this understanding is the fact that scRNA-seq only offers static snapshots of data, since all cells are destroyed upon measurement. Thus it is impossible to monitor how an individual cell changes over time. Moreover, due to the expensive nature of this technology, generally only a handful of discrete timepoints are collected in measuring any differentiation (or state change) process. Finally, the most interesting insights into differentiation are gene regulatory logic that creates state change, and this has proven very difficult to learn using association-based methods (such as mutual information), due noisy measurements and lack of ability to infer causality. 

To address these issues, we take advantage of the recently proposed Neural ODE to model continuous normalizing flows. We treat populations of cells from different time points as samples from distributions over cell states and learn a continuous function that interpolates over time such that the likelihood of data is maximized. Thus we mimic the way cells flow from one state to another during differentiation using a neural network that parameterizes a differential equation. We call this network TrajectoryNet. TrajectoryNet has advantages over existing methods in that it: 

\begin{enumerate}
\item can interpolate by following the manifold of observed entities between measured timepoints, thereby solving the static-snapshot problem, 
\item can create time-continuous trajectories of individual entities,  thus endowing researchers with the ability to follow an entity in time,  
\item forms a deep representational model of system dynamics, which can then be used to understand drivers of dynamics (gene logic in the cellular context), via perturbation of this deep model. 
\end{enumerate}

We note that the key to modeling differentiation is to essentially have the neural network perform a {\em dynamic optimal transport}. We and others  consider optimal transport to likely mimic biology as it is energetically infeasible for cells to take circuitous paths between successive differentiation steps~\cite{hashimoto_learning_2016, schiebinger_optimal-transport_2019, yang_scalable_2019, lederer_emergence_2020}. Thus, we have added penalties to the continuous normalizing flow framework such that it effectively performs dynamic optimal transport of cells.  Our penalties include: 

\begin{enumerate} \item An {\em energy regularization} encouraging lower energy paths in gene space, which we show results in dynamic optimal transport ~\cite{benamou_computational_2000}.

\item A {\em growth rate regularization} that accommodates unbalanced transport. 

\item A {\em density-based penalty} which encourages interpolations that lie on dense regions of the trajectory. 

\item A {\em velocity regularization} where we enforce local estimates of velocity at measured datapoints as given by \citet{la_manno_rna_2018, bergen_generalizing_2019} to match the first time derivative of cell state change.
\end{enumerate}

While we apply this work specifically to cellular dynamics, these penalties can be used in many other situations where we would like to model dynamics based on cross-sectional population level data.



%We note that this does not get around the sample complexity for general empirical distributions \todo{cite} but is not 

%When modeling a continuous time dynamical system using distributional measurements as in scRNA-seq our prior knowledge about the dynamics can most easily be encoded in terms of the paths taken by individual cells. 


==> sections/5_applications.tex <==
scRNA-seq allows sampling the RNA counts of single cells in a sample. Here, we concern ourselves with data collected over a series of discrete timepoints. This data can be particularly helpful in quantifying the heterogeneity between cells within a sample. scRNA-seq is then extremely helpful in examining developing systems with many different cell types. However, scRNA-seq is destructive -- measuring the RNA content of a cell destroys it. Therefore it is not possible to measure a single cell at more than one time. 

However, there are many interesting questions that hinge not on how a population of cells will develop but how an \textit{individual} cell will develop. As such, many methods attempt to infer a global developmental trajectory from this type of data. Early methods fit a prespecified structure, e.g. tree, linear, cyclical, branching etc. to the data. Methods up until now, however, only infer high level and discrete structures. Here we attempt to learn a continuous model of cell state. 

Given a series of single cell measurements over time, we would like to learn a function that given cell state at time $t$, computes cell's development at some time $t+\epsilon$. 

scRNA-seq cannot follow a single cell through development thus making it difficult to infer what transcriptome leads to which eventual adult cell type. However, there are a number of reasonable assumptions on likely trajectories that make inference of cellular lineage possible in an otherwise under defined space. Here, we assume that cells evolve smoothly over time and transcriptional space (and hence can be modelled by ODEs), and that energy is minimized during differentiation such that that cells prefer direct paths  (rather than circuitous paths) towards their eventual states. Finally we assume that the intrinsic space of the cellular transcriptome is a low dimensional manifold, an assumption which repeatedly proven useful in single cell analysis. 

In addition, two extra pieces of information we can obtain directly from the scRNA-sequencing measurements can be translated into further constraints no the transport paths. The first is the RNA-velocity information which gives pointwise $dx/dt$ at each point, and the density at each transcriptional state that can be computed to constrained allowable imbalance in the transport. 
%\begin{enumerate}
 %   \item Cells evolve smoothly over time and transcriptome space and can be modelled with a stochastic differential equation. 
  %  \item Total energy in transcriptome evolution is minimized. Evolution discourages waste of RNA-transcripts, thus any unnecessary transcriptome changes are approximately minimized. 
    
    %\item Cells differentiate primarily based on transcriptome. While there are many factors besides transcriptome that affect differentiation such as chromatin accessability, MicroRNA, and other epigenetics, a majority of these other factors is expressed at some point in the transcriptome~\cite{gulati_single-cell_2020}.
    
   % \item Cell growth / death during development is probabilistic and also minimizes overall transcriptome change. This is assumed in \cite{schiebinger_optimal-transport_2019} and \cite{yang_scalable_2019}.
    %\item We have noisy measurements of $dx/dt$ at all measured cells based on the ratio of spliced to unspliced transcript counts~\cite{la_manno_rna_2018}.
    
    %\item Cell transcriptomes lie in a low dimensional manifold. CITE
%\end{enumerate}

%Smoothness is naturally modelled by a continuous normalizing flow. The energy minimization translates this to a dynamic optimal transport problem. The low dimensional assumption allows us to place an additional cost on paths which deviate from OT, but our assumptions on the underlying dynamics. Finally, we have information about density of different populations $R_{density}$ which will be useful in allowing unbalanced transport and an estimate of $R_{velocity}$ which we can use to enforce realistic path directions.

\input{figures/Tnet_Circle.tex}

\paragraph{Encoding Velocity.} RNA-velocity provides an estimates $\widehat{dx/dt}$ at every measured cell. We use these measurements to regularize the flow direction of flow at every measured cell. Our regularization requires evaluating $f(t,x)$ at periodically at every measured cell adding the regularization:
\begin{align}
    L_{velocity}(t, x, \widehat{dx/dt}) 
    &= \text{cosine-similarity}(f(t,x), \widehat{dx/dt}) \nonumber \\
    &= \frac{f(t,x) \cdot \widehat{dx/dt}}{\left \| f(t,x) \right \| \left \| \widehat{dx/dt} \right \|}
\end{align}
This encourages the direction of the flow at a measured cell to be similar to the direction estimated by RNA-velocity. This ignores the magnitude of the estimate, and only heeds the direction. While RNA-velocity provides some estimate of relative speed, the vector length is considered not as informative, as it is unclear how to normalize these vectors in a system specific way~\cite{la_manno_rna_2018, bergen_generalizing_2019}. We note that while current estimates of velocity can only estimate direction, this does not preclude future methods that can give accurate magnitude estimates. $L_{velocity}$ can easily be adapted to take magnitudes into account by considering $L_2$ similarity for instance.


\paragraph{Encoding the manifold assumption.} Methods that display or perform computations on the cellular manifold often include an implicit or explicit way of normalizing for density and model data gemoetry. PHATE~\cite{moon_visualizing_2019} uses scatterplots and adaptive kernels to display the geometry. SUGAR~\cite{lindenbaum_geometry_2018} explicitly models the data geometry. We would like to constrain our flows to the manifold geometry but not to its density. We penalize the flow such that it is always close to at least a few measured points across all timepoints.
\begin{equation}
    L_{density}(t, x) = \sum_k \max(0, \text{min-k} \bigl ( \left \{ \left \| x(t) - z \right \| : z \in \mathcal{X} \right \} \bigr ) - h)
\end{equation}
This can be thought of as a loss which penalizes points until they are within $h$ euclidean distance of their $k$ nearest neighbors. We use $h=0.1$ and $k=5$ in all of our experiments. We evaluate $L_{density}$ on an interpolated time $t_d \in (t_0, t_k)$ every batch. 

\input{figures/growth.tex}

==> tables/eb_table_v4.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &    t=1 &    t=2 &    t=3 &   mean \\
\midrule
Base     &  0.764 &  0.811 &  0.863 &  0.813 \\
Base + D &  0.759 &  0.783 &  0.811 &  0.784 \\
\midrule
OT       &  0.791 &  0.831 &  0.841 &  0.821 \\
prev     &  1.715 &  1.400 &  0.814 &  1.309 \\
next     &  1.400 &  0.814 &  1.694 &  1.302 \\
rand     &  0.872 &  1.036 &  0.998 &  0.969 \\
\bottomrule
\end{tabular}


==> tables/eb_table_v6.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &    t=1 &    t=2 &    t=3 &   mean \\
\midrule
Base         &  0.764 &  0.811 &  0.863 &  0.813 \\
Base + D     &  0.759 &  0.783 &  0.811 &  0.784 \\
Base + V     &  0.816 &  0.839 &  0.865 &  0.840 \\
Base + D + V &  0.930 &  0.806 &  0.810 &  0.848 \\
Base + E     &  0.737 &  0.896 &  0.842 &  0.825 \\
Base + G     &  0.700 &  0.913 &  0.829 &  0.814 \\
prev         &  1.715 &  1.400 &  0.814 &  1.309 \\
next         &  1.400 &  0.814 &  1.694 &  1.302 \\
OT           &  0.791 &  0.831 &  0.841 &  0.821 \\
rand         &  0.872 &  1.036 &  0.998 &  0.969 \\
\bottomrule
\end{tabular}


==> tables/generated_full_v2.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{3}{l}{emd} & \multicolumn{3}{l}{mse} \\
{} &   Arch &  Cycle &   Tree &   Arch &  Cycle &   Tree \\
\midrule
Base         &  0.691 &  0.037 &  0.490 &  0.300 &  0.190 &  0.218 \\
Base + D     &  0.607 &  0.049 &  0.373 &  0.236 &  0.191 &  0.145 \\
Base + V     &  0.243 &  0.033 &  0.143 &  0.107 &  0.068 &  0.098 \\
Base + D + V &  0.415 &  0.034 &  0.252 &  0.156 &  0.081 &  0.132 \\
prev         &  1.086 &  0.035 &  1.092 &  0.652 &  0.192 &  0.666 \\
next         &  1.090 &  0.035 &  1.068 &  0.659 &  0.192 &  0.689 \\
OT           &  0.644 &  0.032 &  0.492 &  0.252 &  0.192 &  0.196 \\
rand         &  0.622 &  0.406 &  0.420 &  0.243 &  0.346 &  0.161 \\
\bottomrule
\end{tabular}


==> tables/kantorovich_table_v3.tex <==
\begin{table}[hbt]
    \centering
\begin{tabular}{lrrrr}
\toprule
{} &    t=1 &    t=2 &    t=3 &   mean \\
\midrule
Base          &  0.606 &  0.505 &  0.572 &  0.561 \\
Base + D      &  0.499 &  0.562 &  0.459 &  0.507 \\
Base + D + V  &  \textbf{0.421} &  \textbf{0.382} &  0.497 &  \textbf{0.433} \\
\midrule
OT            &  0.529 &  0.420 &  0.510 &  0.486 \\
prev          &  1.905 &  1.071 &  \textbf{0.406} &  1.127 \\
next          &  1.071 &  0.406 &  0.607 &  0.695 \\
rand          &  0.749 &  0.654 &  0.545 &  0.649 \\
\bottomrule
\end{tabular}
 \caption{Shows the Wasserstein distance (EMD) between the left out timepoint and the predicted distribution for various methods on the 5 timepoint embryoid body dataset.}
    \label{tab:eb_comparison_table}
\end{table}


==> tables/noonan_table_v3.tex <==
\begin{tabular}{llll}
\toprule
{} &              rep1 &              rep2 &              mean \\
\midrule
Base         &  0.888 $\pm$ 0.07 &  0.905 $\pm$ 0.06 &  0.897 $\pm$ 0.06 \\
Base + D     &  0.882 $\pm$ 0.03 &  0.895 $\pm$ 0.03 &  0.888 $\pm$ 0.03 \\
Base + D + V &  \textbf{0.839} $\pm$ 0.06 &  \textbf{0.862} $\pm$ 0.04 &  \textbf{0.851} $\pm$ 0.05 \\
\midrule
OT           &             1.098 &             1.095 &             1.096 \\
prev         &             1.628 &             1.573 &               1.6 \\
next         &             1.324 &             1.391 &             1.357 \\
rand         &             1.333 &             1.288 &             1.311 \\
\bottomrule
\end{tabular}

